A Smoothed Dual Approach for Variational Wasserstein Problems

Variational problems that involve Wasserstein distances have been recently proposed to summarize and learn from probability measures. Despite being conceptually simple, such problems are computationally challenging because they involve minimizing over quantities (Wasserstein distances) that are themselves hard to compute. We show that the dual formulation of Wasserstein variational problems introduced recently by Carlier et al. (2014) can be regularized using an entropic smoothing, which leads to smooth, differentiable, convex optimization problems that are simpler to implement and numerically more stable. We illustrate the versatility of this approach by applying it to the computation of Wasserstein barycenters and gradient flows of spacial regularization functionals.

==> sections/old/old-extensions.tex <==
In order to enforce additional properties of the barycenters, it is possible to penalize~\eqref{eq-variational-barycenter-discrete} with an additional convex regularization $J$, which reads
\eql{\label{eq-bary-penalized}
	\umin{\p \in \Si_d} \sum_{k=1}^K \la_k  H_{q_k}(\p) + J(\p).
}
The following proposition, whose proof is similar as the one of Theorem~\ref{prop-dual-energy} provides an explicit formulation of the dual of that program:

\begin{proposition}
	The solution $p^\star$ solving~\eqref{eq-bary-penalized} satisfies~\eqref{eq-primal-dual-relationship} where $( g_k^\star )_k$ are any solution of the following dual problem
	\eql{\label{eq-dual-penalized}
		\umin{ g_1,\ldots, g_K} \sum_{k} \la_k H_{\q_k}^*(g_k)
			+ J^*\bpa{ \sum_k \la_k g_k }
	}
\end{proposition}

When $J=0$, that is no regularizer on $\p$ is added, one obtains $J^* = \iota_{\{0\}}$, which is equivalent to the original formulation in Eq.~\eqref{eq-dual-pbm}. Relevant examples of penalizations $J$ include:
\begin{itemize}
	\item In order to enforce some spread of the barycenter, one can use $J(p) = \frac{\ga}{2}\norm{p}^2$, in which case $J^*(g) = \frac{1}{2\ga}\norm{g}^2$. In contrast to~\eqref{eq-dual-pbm}, the dual problem~\eqref{eq-dual-penalized} is now an unconstraint smooth optimization. This problem can be solved using a simple Newton descent.  
	\item One can also enforce that the barycenter entries are smaller than some maximum value $\rho$ by setting $J = \iota_{\Cc}$ where $\Cc = \enscond{p}{\normi{p} \leq \rho}$. In this case, one has $J^*(g) = \rho \norm{g}_1$. The optimization~\eqref{eq-dual-penalized} is now an unconstrained non-smooth optimization. Since the penalization is an $\ell^1$ norm, one solve it using first order proximal methods. %\todo{see how to detail this, if needed}.  
	\item To force the barycenter to assume some fixed values $p_I^0 \in \RR^{|I|}$ on a given set $I$ of indices, one can use $J=\iota_{\Cc}$ where $\Cc = \enscond{p}{p_I = p_I^0}$ where $p_I=(p_i)_{i \in I}$. One then has $J^*(g) = \dotp{g_I}{p_I^0} + \iota_{\{0\}}(g_{I^c})$ %\todo{check this}.
\end{itemize}

==> sections/old/old-newton.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \subsection{Implementation of Second Order Approaches}
 
 It is also possible to use more advanced optimization schemes to compute descent directions: since the problem we consider has a convex objective of $nN$ variables, is differentiable and has $n$ equality constraints, one can use generic toolboxes that only require first order information, such as the the \texttt{fmincon} matlab function. Moreover, since $H_{\p_k}^*$ is $C^2$ and its Hessian is defined in Eq.~\eqref{eq-hessien-dual}, we can also use a Newton descent constrained to the affine space $\enscond{ (g_k)_k }{ \sum_k \la_k g_k = 0 }$~\cite[\S10]{Boyd:1072}. This method is more costly, but can be still carried out effectively. For the sake of completeness, we provide additional details on this approach below.
 
 \subsection{Newton Method with Equality Constraints}
 
 This approach can be carried out by solving at each gradient iteration a linear KKT system: writing $\Delta$ for the $n\times N$ matrix of gradients as described in Eq.~\eqref{eq:onehistograd}, where each column $\Delta_k$ is equal to the gradient of $H^*_{\q_k}$ computed at $g_k$, computing the Newton descent directions requires solving a symmetric indefinite linear system in the Newton steps $\Delta_k^\text{nt}$ and the additional Lagrange multiplier variable $\rho \in \RR^n$:
 \begin{equation}\label{eq:newton}
 \begin{bmatrix} \nabla^2 H^*_{q_1}(g_1) & \zeros & \cdots & \zeros & \lambda_1 I_n \\ \zeros & \nabla^2 H^*_{q_2}(g_2) & \zeros & \zeros & \lambda_2 I_n \\ \vdots & \ddots& \ddots &  \vdots & \vdots \\ \zeros & \cdots & \zeros &   \nabla^2 H^*_{q_N}(g_N) & \lambda_N I_n \\\lambda_1 I_n & \cdots & \cdots & \lambda_N I_n & \zeros_{n\times n}\end{bmatrix} \begin{bmatrix}\Delta^{\text{nt}}_1 \\ \Delta^{\text{nt}}_2 \\ \vdots \\ \Delta^{\text{nt}}_N \\ \rho \end{bmatrix}= \begin{bmatrix}\Delta_1 \\ \Delta_2 \\ \vdots \\ \Delta_N \\ \zeros_n \end{bmatrix}.
 \end{equation}
 
 % \eq{
 % 	\foralls k \in N, \quad \IT{H_k} g_k + h = -\IT{v_k}, 
 % 	\qandq
 % 	\sum_k \la_k g_k = 0.
 % }
 \subsection{Truncated Newton and Regularization} The truncated Newton approach~\cite{nash2000survey} consists in approximating the computation of the Newton direction by solving only approximately that linear system with a few conjugate gradient steps. To do so, we can consider the three following arguments:
 
 A conjugate gradient approach to solve Eq.~\eqref{eq:newton} involves the repeated application of the KKT linear map of dimension $n(N+1)\times n(N+1)$, as described in the left-hand side of Eq.~\eqref{eq:newton}, to a running estimate of the solution. In practice, that map can be implemented using Schur products and two matrix-matrix products that only involve a $(n\times n)$ matrix $K$ and another of size $n\times N$, as shown in Eq.~\eqref{eq:onehistohessian}.
 
 Because for any histogram $q$ the Hessian of $H^*_q$ is rank deficient---Eq.~\eqref{eq:onehistograd} shows that the gradient of $H^*_q$ is invariant under the element-wise addition of a constant to $g$, therefore the vector $\ones_n$ is in the null space of $\nabla^2 H^\star_q(g)$---the linear system in Eq.~\eqref{eq:newton} is rank deficient as well. This problem can be solved by regularizing each Hessian in that matrix with a constant $\varepsilon$ times the identity. In all our experiments, this constant has been set to $\varepsilon=\frac{1e-2}{n\gamma}$. Algorithmically, this is equivalent to adding the matrix $\varepsilon X$ to the matrix $\nabla^2H^* X$ in Eq.~\eqref{eq:onehistohessian} at each conjugate gradient iteration. 
 
 Finally, choosing a pre-conditioner that reduces the conditioning number of the KKT system of Eq.~\eqref{eq:newton} can  prove beneficial to solve it faster. We propose to approximate each Hessian sub-matrix $\nabla^2 H^*_{q_k}(g_k)$ in the KKT system of Eq.~\eqref{eq:newton} by the diagonal matrix formed with its gradient, which is the leading term on the right-hand-side of Eq.~\eqref{eq-hessien-dual}. We form a left-preconditioner matrix $P$ of size $(N+1)n\times (N+1)n$ by substituting to each Hessian in Eq.~\eqref{eq:newton} this diagonal approximation while still adding, as mentioned above, a regularizer $\varepsilon$. $P$ can be expprop-dual-energylicitly inverted using the block-wise matrix inversion lemma. Rather than writing down this matrix here, we simply write in Eq.~\eqref{eq:precond} and in the spirit of Eq.~\eqref{eq:onehistohessian}, the result of the application of $P^{-1}$ on the $n\times \N$ matrix $X$ of direction variables as well as the update of the Lagrangean multiplier vector $\rho$. Using the auxiliary variables
 
 $$\tilde{\Delta}=\frac{\ga}{\Delta+\varepsilon \ones_{n\times N}};\quad \tilde{\Delta}_\lambda= \tilde{\Delta}\diag(\lambda),\quad r=\frac{1}{\tilde{\Delta}\left(\lambda \circ \lambda\right)}, \quad\tilde{r}=r\circ\left((X\circ\tilde{\Delta})\lambda\right)$$
 this update results in
 \begin{equation}\label{eq:precond}\begin{aligned}
 X &\leftarrow \ga X/\Delta+\tilde{\Delta}_\lambda \diag(r\circ\rho-\tilde{r}),\\
 \rho &\leftarrow \tilde{r}-r\circ\rho.
 \end{aligned}\end{equation}
 	
 	
 	% 
 	% \frac{1}{\gamma} \left[\Delta\circ X - A \circ \left(K  \left(\frac{Q\circ \left(K \left(A\circ X\right)\right)}{B\circ B} \right)\right) \right].\end{aligned}\end{equation}
 
 
 % 
 % 
 % \begin{algorithm}
 % 	\begin{algorithmic}[1]
 % 		\caption{Second Order Method\label{algo:newton}}
 % 		\STATE \textbf{Input}: $Q=[\q_1,\cdots,\q_N] \in(\Sigma_n)^N$, metric $M\in\RR_+^{n\times n}$,$\lambda\in\Sigma_N$, $\gamma>0$, stepsize $\tau>0$. 
 % 		\STATE initialize $G\in\mathbb{R}^{n\times N}$ and form the $n\times n$ matrix $K=e^{-M/\gamma }$.
 % 		\REPEAT
 % 				\STATE{Compute gradient matrix $\Delta$, see Eq.~\eqref{eq:onehistograd}.}
 % 				\STATE{Solve to desired precision the KKT system of Eq.~\eqref{eq:newton} using an iterative linear system solver and a pre-conditioner to obtain a $n\times N$ matrix of approximate Newton descent directions $\Delta^{\text{nt}}$.}
 % 				\STATE $G = G - \tau \Delta^{\text{nt}}$ (gradient update  with approximate line search to set $\tau$.)
 % 				\STATE $G = G - \frac{1}{\norm{\lambda}_2^2}(G \lambda)  \lambda^T$ \quad (projection such that $G\lambda=0$)
 % 		\UNTIL{$\ones_d^T\sqrt{(Z\circ Z) \ones_N/N}<\varepsilon$, where $Z=\Delta(I_N-\frac{1}{N}\ones_N\ones_N^T)$}
 % 		\STATE output barycenter $\p=\Delta \ones_N/N$.
 % 	\end{algorithmic}
 % \end{algorithm}


==> sections/old/old-wasserstein-propagation.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Wasserstein Propagation}

The dual approach can be easily extended to more complicated convex functionals involving Wasserstein distances. To illustrate this, we show how the Wassertein propagation problem introduced by~\cite{Solomon-ICML} can be solved efficiently with our approach. This problem considers a graph with nodes indexed by $\Nn = \Nn_S \cup \Nn_T$. Here $t \in \Nn_T$ indexes boundary nodes where fixed input distributions $p_t \in \RR^N$ are defined. The goal is to propagate these histograms to the inner nodes $s \in \Nn_S$ to compute inner histograms $p_s \in \Sigma_n$
\eql{\label{eq-wass-propagation}
	\umin{ (p_s)_{s \in \Nn_S} }
		\sum_{ (s,t) \in \Ee_{S,T} }  \la_{s,t} W(p_s,q_t)
		+ 
		\sum_{ (s,s') \in \Ee_{S} }  \la_{s,s'} W(p_s,p_{s'})
}
where $\la_{s,t} \geq 0$ are weights, and $\Ee_{S,T}$ denotes the set of (non-directed) edges between nodes of $\Nn_S$ and $\Nn_T$, and $\Ee_S$ denoted interior edges between two nodes of $\Nn_S$. Similarly to the approach outlined in Theorem~\ref{prop-dual-energy}, we define a dual optimization problem by introducing, for each interior index $s$, duplicated histograms $h_{s,e} \in \Si_n$ and the corresponding dual variable $g_{s,e} \in \RR^N$ for each edge $e=(s,t) \in \Ee_{S,T} \cup \Ee_S$ which we denote as $e \supset s$. The dual problem amounts to solving:
\eq{
	\umin{ (g_{s,e})_{s \in \Nn_s}^{e \supset s} }
		\sum_{ e=(s,t) \in \Ee_{S,T} }  \la_{s,t} H_{q_t}^*(g_{s,e})
		+ 
		\sum_{ e=(s,s') \in \Ee_{S} } \la_{s,s'} W^*(g_{s,e},g_{s',e})
}
\eq{
	\qstq	\foralls s \in \Nn_S, \quad \sum_{e=(s,t) \supset s} \la_{s,t} g_{s,e} = 0.
}
The primal variables are then retrieved by the relationships
\eq{
	\foralls (s,t) \in \Ee_{S,T}, \; p_s = \nabla H_{q_t}^*(g_{s,e}), 
	\qandq
	\foralls e=(s,s') \in \Ee_{S}, \; (p_s,p_s') = \nabla W_{\ga}^*(g_{s,e},g_{s',e}).	
}



%%%
\paragraph{Wasserstein Propagation}

The Wassertein propagation problem introduced in~\cite{Solomon-ICML} considers histograms $(p_t)_{t \in \Nn}$ indexed by nodes $\Nn$ of a weighted graph, where $\la_{t,t'} > 0$ if there is an edge $(t,t') \in \Nn \times \Nn$. These histograms solve
\eql{\label{eq-wass-propag}
	\umin{(p_t)_t} \sum_{t \sim t'} \la_{t,t'} W(p_t,p_t')
	\quad\text{subj. to}\quad
	\foralls t \in \tilde\Nn, \quad p_t = q_t,
}
where $\tilde\Nn \subset \Nn$ indexes a set of prescribed input histograms $(q_t)_{t \in \tilde\Nn}$. 
The barycenter problem~\eqref{eq-variational-barycenter-discrete} is a special case with only a single free variable and a star-like graph.
%
It is possible to define a dual problem where the dual variables are indexed by the edge of the graph. The dual objective function is a sum of Legendre transforms of $W$ with respect to both variables, as defined in~\eqref{eq-dfn-dual-bothvar}. It is thus possible to solve~\eqref{eq-wass-propag} using a projected gradient descent thanks to the closed form expression~\eqref{eq-grad-bothvar} for the gradient.




==> sections/old/removed.tex <==


%% I PUT HERE STUFF REMOVED %%%
\if 0
\subsection{Constrained Newton Algorithm}

To obtain faster quadratic convergence, one can make use of the second order information through a constrained Newton update step
\eq{
	( \IIT{g_{k}} )_{k} = \uargmin{ (g_k)_k } 
	\sum_{k}  \la_k \pa{ \dotp{ \IT{v_k} }{ g_k }
			+ \frac{1}{2} \dotp{ \IT{H_k} g_k }{ g_k }  }
		\qstq \sum_k \la_k g_k = 0.			
}
where $\IT{v_k} = \nabla H_{q_k}^*( \IT{g_k} )$ and $\IT{H_k} = \partial^2 H_{q_k}^*( \IT{g_k} )$. This update thus requires the resolution of the following symmetric linear system in $(g_k)_k$ and the additional Lagrange multiplier variable $h \in \RR^q$
\eq{
	\foralls k \in K, \quad \IT{H_k} g_k + h = -\IT{v_k}, 
	\qandq
	\sum_k \la_k g_k = 0.
}
In practice, one performs a truncated Newton iteration by perform a few conjugate gradient steps. The computation of $\IT{v_k}$ and the application of $\IT{H_k}$ to a vector are carried over by performing soft nearest neighbors assignments as defined by formula~\eqref{eq-gradient-dual}. The number of conjugate gradient step can be monitored to ensure a sufficient decay of the primal energy. 

%%%
\subsection{[tentative idea] Parameterized Barycenters}

We seek here a barycenter which a (linear) combination of a few atoms $(p_i)_{i \in I}$ where $p_i \in \Si_n$, and thus consider
\eq{
	\foralls u \in \RR^I, \quad P(u) = \sum_{i in I} u_i p_i.
}
We assume here that $P$ is injective, i.e. the atoms forms a basis of $\Im(P)$. Writing $p=P(u)$ in~\eqref{eq-variational-barycenter-discrete} leads to consider the strictly convex program
\eq{
   \umin{u \in \Si_I} \sum_k \lambda_k W( P(u), q_k ).
}
Problem: how to compute $(H_q \circ P)^*$ as a function of $H_q^*$ ? Not trivial because $P$ is nos surjective. 


%%%
\subsection{[tentative] Generic Framework }

We consider problem of the form
\eql{\label{eq-optim-generic}
	\umin{u \in \Si_I} \phi\pa{ ( W(P(u),q_k) )_{k=1}^K }
}
where $\phi : \RR^K \rightarrow \RR$ is convex and increasing in each of its argument, so that~\eqref{eq-optim-generic} is a convex problem.
\fi

==> sections/old/sec-dictionary-learning-new-experiments.tex <==
\subsection{Learning parts of smileys}

We applied our method to a toy database of simley faces that we generated with a circle as the contour of the face and different kinds of eyes and mouths, shifted up to 8 pixels horizontally and vertically (Figure \ref{fig:smileyData}). The distance between two pixels is take to be the euclidean distance between their position. The results, shown in Figure \ref{fig:smileyLearned}, seem to indicate that the wasserstein cost is more able to isolate individual parts than the Kullback-Liebler cost.

\begin{figure}[ht]
\center\includegraphics[width=.55\textwidth]{img/Smileys_basis.png}
\includegraphics[width=.15\textwidth]{img/Smileys_data.png}
\label{ig:smileyLearned}
\caption{(Left) Basic elements for making smiley faces. (Right) Three examples of generated smileys}
\end{figure}

\begin{figure}[ht]
\center\includegraphics[width=.45\textwidth]{img/Smiley_dictionary_KL.png}
\hspace{.08\linewidth}
\includegraphics[width=.45\textwidth]{img/Smiley_dictionary_wass.png}
\label{ig:smileyLearned}
\caption{(Left) Dictionary learned by NMF with a KL divergence cost. (Right) Dictionary learned with our method}
\end{figure}

\subsection{Learning color palettes}

We also applied our method to color histograms of images, in order to learn basic color palettes. We used the Oxford flower database and applied the following preprocessing: we mapped the images to their chrominance in the YUV space (the U and V channels), then quantized the colors appearing in the database using k-means to obtain histograms. We took the distance between to bins in a histogram as the distance between the corresponding cluster means in the chrominance space. Figure \ref{fig:colorPalettes} shows the results of this experiment. Each palette has a dominant color, which could correspond to the color palette of a specific kind of flower or of a kind of background (grass, gravel\dots).

%\begin{figure}[ht]
%\includegraphics[width=.9\textwidth]{img/palettes_naive_10.png}
%\label{ig:colorPalettes}
%\caption{10 palettes learning with our method. Each color in a palette is represented by a point on its (U,V) coordinates whose size is positively linked to its weight in the palette}
%\end{figure}

\begin{figure}[ht]
\includegraphics[width=.9\textwidth]{img/palettes_10.png}
\label{ig:colorPalettes}
\caption{10 palettes learning with our method. Each color in a palette is represented by a 20-by-20 image in which each of the 400 pixels was sampled iid from the probability distribution represented by the palette's histogram}
\end{figure}






==> sections/old/sec-dictionary_learning.tex <==
\section{Dictionary learning with smooth Wasserstein fitting cost}\label{sec:nmf}
We illustrate in this section the versatility of Theorem~\ref{prop-dual-energy}, and how it can be adapted to carry out dictionary learning with a Wasserstein reconstruction error on a dataset of histograms arranged as a $n\times N$ matrix $Q=[q_1,\cdots,q_N]$.

\paragraph{Problem Formulation}
The dictionary learning problem with Wasserstein fitting cost consists in learning simultaneously $m$ dictionary elements and $N$ vectors of weights in $\Sigma_m$ to reconstruct each of the original histograms as a linear combination of the dictionary elements, namely find a dictionary $D$ and weights $\Lambda$ such that
\begin{equation}
\label{eq:DL} 
\begin{tabular}{ll}
$\displaystyle\min_{D\in\mathbb{R}^{n\times m},\Lambda\in\mathbb{R}^{m\times N}}$& $\displaystyle\sum_{k=1}^N H_{q_k}(D\lambda_k)$
\end{tabular}
\end{equation}
with the implicit constraint that $D\Lambda\in\Sigma_n^N$. 

\paragraph{Previous work} This problem was previously considered by \cite{sandler2009} and \cite{zen2014simultaneous}. \cite{sandler2009} rely on a fast approximation of optimal transport that uses Wavelet decompositions \cite{shirdhonkar2008approximate} but which only works in practice when $\Xcal$ is $\RR^2$ or $\RR^3$. \cite{zen2014simultaneous} propose a similar matrix factorization and approach while also learning a cost matrix $M$ (not necessarily a metric) using labels. Their formulation relies on large-scale linear programs (not network flows) whose complexity grows very quickly with the relevant dimensions $m,N$ and $n$ of the problem. Our approach is not restricted to particular choices for $\Xcal$ and can scale to large dimensions/datasets/dictionary sizes: we do make any assumption on the metric space $(\Xcal,D)$ other that the $n^2$ matrix of pairwise distances between the $n$ points in $\Xcal$ can be stored in memory. This versatility is illustrated  in our experiments below, in which we carry out Wasserstein NMF on texts seen as large clouds of points in $\RR^{50}$ using word embeddings~\cite{pennington2014glove,zou2013}.

\paragraph{Dual formulation} Let $D^\star_\Lambda$ (resp. $\Lambda^\star_D$) be the solution of (\ref{eq:DL}) with $\Lambda$ (resp. $D$) fixed. The following theorem links $D^\star_\Lambda$ (resp. $\Lambda^\star_D$) and $\Lambda$ (resp. $D$) when the rank of $\Lambda$ (resp. $D$) is $m$.

\begin{theorem}
$\Lambda^\star_D$ can be computed as $D\lambda^\star_{Di}=\nabla H^*_{q_k}(g^{\star\Lambda}_i)$ where and $(g^{\star\Lambda}_i)_{i=m}^n$ is the solution of
\begin{equation*}
\label{eq:lambdaSubProblems}
\displaystyle\min_{D^Tg_k=0} H^*_{q_k}(g_k)\,,\quad k=1\cdots N
\end{equation*}
Furthermore $D^\star_\Lambda$ can be computed as \\$D^\star_\Lambda=(\nabla H^*_{q_k}(g^{\star D}_i))_{k=1\cdots N}$ where $G^{\star D}$ is the solution of
\begin{equation*}
\displaystyle\min_{G\Lambda^T=0} \sum_{k=1}^N H^*_{q_k}(g_k)
\end{equation*}
\end{theorem}
The proof is almost identical to that of \ref{prop-dual-energy} and left out for lack of space.

When $D$ is fixed, $\Lambda^\star_D$ can be computed with Algorithm \ref{algo:firstorder} by replacing the projection step by $G=G-GDD^+$ where $D^+$ is the peudo-inverse of $D$, and the output is $\Lambda^\star_D= D^+\nabla H^*_Q(G)$. Similarily when $\Lambda$ is fixed, $D^\star_\Lambda$ can be computed with Algorithm \ref{algo:firstorder}  by replacing the projection by $G=G-\Lambda^+\Lambda G$, and the output is $D^\star_\Lambda= \nabla H^*_Q(G)\Lambda^+$.

We can minimize Eq.~\eqref{eq:DL} using alternated optimization. Our algorithm gains numerical stability when the columns of $D$ and $\Lambda$ are projected on the simplex (of size $n$ and $m$) at each iteration.

Note that if $D_0^T\mathbf{1}=\mathbf{1}$ and the rank of $\Lambda$ (resp. $D^T$) stays equal to $m$, $D^{\star T}_\Lambda\mathbf{1}=\mathbf{1}$ (resp. $\Lambda^{\star T}_D\mathbf{1}=\mathbf{1}$). 

\paragraph{Experiments on synthetic data}
In this experiment with toy-data, we consider an input matrix $Q$ using 3 Gaussians centered around $-6$, $0$ and $6$ and with variance $2$, discretized on $[-12, 12]$ with $401$ evenly spaced points. Each column of $Q$ is generated as a weighted sum of those gaussians with a shift on the means. The weights (resp. shifts) are evenly distributed on $[0, 1]$ (resp. $[-2, 2]$) and each resulting vector is normalized so that its coordinates sum to one (examples of such histograms are provided in the top right part of Figure \ref{fig:k3}). We generate $N=1000$ histograms that way. The lower half of Figure \ref{fig:k3} displays dictionary learned under the Wasserstein metric with our approach (smoothing parameter $\gamma=1/50$) and the standard NMF algorithm with multiplicative updates and KL fitting cost~\cite{lee1999learning}. These computations require less than a few minutes on a desktop machine.

\begin{figure}[!h]
        \centering
        \includegraphics[width=.235\textwidth]{Synthetic_basis}
        \includegraphics[width=.235\textwidth]{Synthetic_ex4}
        \includegraphics[width=.235\textwidth]{Synthetic_WNMF_k3_lambda100}
        \includegraphics[width=.235\textwidth]{Synthetic_NMF_k3}
        \caption{(top left) gaussians used to generate the data (top right) 4 examples of histograms generated using random shifts and weights. We use $N=1000$ histograms to learn a dictionary using either: (bottom left) our algorithm with Wasserstein fitting cost with $m=3$ dictionary elements and $\gamma=1/50$; (bottom right) a KL fitting cost with $m=3$.}
        \label{fig:k3}
\end{figure}


\paragraph{Translingual Topic Modeling}
We consider the problem of summarizing a set of texts seen as bags-of-words in a given language as a convex combinations of topics (bags-of-words) in a different language. To carry out such a task with optimal transport, we need a metric between words in both languages. This metric can be defined using \cite{zou2013}'s work, which proposes a bilingual embedding of both English and Chinese words in $\Xcal=\RR^{50}$. The Euclidean metric between such embeddings can be used directly to define the cost matrix $M$, with an exponent $\rho=1$. In this setting $n$, the total number of points, is equal to $n_E+n_C$ where $n_E$ (resp. $n_C$) is the size of the English (resp. Chinese) dictionary considered for such texts.

We applied our Wasserstein-NMF method to a all 10788 English texts taken from the reuters corpus. We remove common english stop-words and words that are not in the word embedding dictionary of~\cite{zou2013} to obtain dictionary sizes of $n_E=11978$ English words and $n_C = 4070$ Chinese words. We set $m=6$, $\gamma=\frac{1}{50}$ and we learn dictionary elements with the constraint that they are exclusively supported on the $n_C$ bins that correspond to \textbf{Chinese words}, namely we wish to reconstruct each English text (seen as a bag-of-English-words) using convex combinations of bags-of-Chinese-words. We display the first factor computed by our method in Figure \ref{fig:mandarin} as a cloud-of-words, where each word's size is proportional to its frequency, and only the most frequent words are reported. That topic is dominated by words (single Chinese characters or pairs) related to international trade.

\begin{figure}[!h]
        \centering
        \includegraphics[height=.5\textwidth, angle=270]{Mandarin3}
\caption{Wordle representation of 1 of the 6 mandarin topics learned for $\gamma=1/50$. Only the 50 most frequent words are represented. The font size increases monotonically with the word frequency}\label{fig:mandarin}
\end{figure}

==> sections/sec-regularized-barycenters2.tex <==
% !TEX root = ../WassersteinDual.tex

%%%%%%%%%%%%%%%%
\section{Regularized Problems}
\label{sec:exten}

We show in this section that our dual optimization framework is versatile enough to deal with functionals involving Wasserstein distances that are more general than the initial WBP problem.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Regularized Wasserstein Barycenters}\label{sec:regularized}

In order to enforce additional properties of the barycenters, it is possible to penalize~\eqref{eq-variational-barycenter-discrete} with an additional convex regularization, and consider
\eql{\label{eq-regul-primal}
	\umin{p} \sum_{k=1}^N w_k H_{q_k}(p) + J(\Aa p),
}
where $J$ is a convex real-valued function, and $\Aa$ is a linear operator.

The following proposition shows how to compute such a regularized barycenter through a dual optimization problem. 

\begin{prop}
The dual problem to~\eqref{eq-regul-primal} reads
\eql{\label{eq-regul-dual}
	\umin{(u_k)_{k=1}^N, v} \sum_{k=1}^N w_i H_{q_k}^*(u_k) + J^*(v) + \iota_{H}(v,(u_k)_k)
}
\eq{
	\qwhereq
	H \eqdef \enscond{ ((u_k)_{k=1}^N, v) }{ \Aa^* v + \sum_k w_k u_k = 0 },
}
and the primal-dual relationships read
\eql{\label{eq-primal-dual}
	\foralls k=1,\ldots,N, \quad p = \nabla H_{q_k}^*(u_k). 
}
\end{prop}

\begin{proof}
	We re-write the initial program~\eqref{eq-regul-primal} as 
	\eql{\label{eq-primal-reformulated}
		\umin{\pi} F( B\pi ) + G(\pi)
	} 
	where we denoted, for $\pi=(p,p_1,\ldots,p_N)$, 
	\begin{align*}
			B \pi &\eqdef (\Aa p, p, p_1,\ldots,p_N) \\
			F(\beta,q, p_1,\ldots,p_N) &\eqdef J(\beta) + \iota_{C}(q,p_1,\ldots,p_N),\\
			G(p, p_1,\ldots,p_N) &\eqdef \sum_k w_k H_{q_k}(p_k)
	\end{align*} 
	for $C \eqdef \enscond{(q,p_1,\ldots,p_N)}{\forall k, p_k=q}$.
	%
	The Fenchel-Rockafelear dual to~\eqref{eq-primal-reformulated} reads
	\eq{
		\umax{\nu = \{v,u,(u_k)_k\}} - F^*(\nu) - G^*(-B^* \nu) 
	}
	where 
	\begin{align*}
		G^*(u,u_1,\ldots,u_N) &= \sum_k w_k H_{q_k}^*(u_k/w_k) + \iota_{\{0\}}( u ),  \\
		B^*(\nu) &= (\Aa^* v + u, u_1,\ldots,u_N), \\
		F^*(\nu) &= J^*(v) + \iota_{C^\bot}(u,u_1,\ldots,u_N), 
	\end{align*} 
	where $C^\bot = \enscond{ (u,u_1,\ldots,u_N) }{u + \sum_k u_k=0}$. 
	One thus obtains the dual
	\eq{
		\umin{ v,b,(u_k)_k } \sum_k w_k H_{q_k}^*(-u_k/w_k)
		\qstq
		\choice{
				\Aa^* v + u = 0, \\
				u + \sum_k u_k=0.
		}
	}	
	The primal-dual relationships reads $\pi \in \partial G^*(-B^* \nu)$, and hence~\eqref{eq-primal-dual}. 
	Changing $-u_k/w_k$ into $u_k$ give the desired formula. 
\end{proof}

Relevant examples of penalizations $J$ include:
\begin{itemize}
	\item In order to enforce some spread of the barycenter, one can use $\Aa=\Id$ and $J(p) = \frac{\la}{2}\norm{p}^2$, in which case $J^*(g) = \frac{1}{2 \la}\norm{g}^2$. In contrast to~\eqref{eq-dual-pbm}, the dual problem~\eqref{eq-regul-dual} is equivalent to an unconstraint smooth optimization. This problem can be solved using a simple Newton descent.  
	\item One can also enforce that the barycenter entries are smaller than some maximum value $\rho$ by setting $\Aa=\Id$ and $J = \iota_{\Cc}$ where $\Cc = \enscond{p}{\normi{p} \leq \rho}$. In this case, one has $J^*(g) = \rho \norm{g}_1$. The optimization~\eqref{eq-regul-dual} is equivalent an unconstrained non-smooth optimization. Since the penalization is an $\ell^1$ norm, one solve it using first order proximal methods as detailed in Section~\ref{sec-first-order-split} bellow.
	\item To force the barycenter to assume some fixed values $p_I^0 \in \RR^{|I|}$ on a given set $I$ of indices, one can use $\Aa=\Id$ and $J=\iota_{\Cc}$ where $\Cc = \enscond{p}{p_I = p_I^0}$ where $p_I=(p_i)_{i \in I}$. One then has $J^*(g) = \dotp{g_I}{p_I^0} + \iota_{\{0\}}(g_{I^c})$.
	\item To force the barycenter to have some smoothness, one can select $\Aa$ to be a spacial derivative operator (for instance a gradient approximated on some grid or mesh) and $J$ to be a norm such as an $\ell^2$ norm (to ensure uniform smoothness) or an $\ell^1$ norm (to ensure piecewise regularity). We explore this idea in Section~\ref{sec-tv-regul}.  
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Resolution using First Order Proximal Splitting}
\label{sec-first-order-split}

Assuming without loss of generality that $w_N \neq 0$ (otherwise one simply needs to permute the ordering of the input densities), one can note that it is possible to remove $u_K$ from~\eqref{eq-regul-dual} by imposing, for $x = ((u_k)_{k=1}^{N-1}, v)$
\eq{
	u_N(x) \eqdef - \frac{\Aa^*v}{w_N} - \sum_{i=1}^{N-1} \frac{w_k}{w_N}  u_k, 
} 
and then one can consider the following optimization problem without the $H$ constraint
\eql{\label{eq-primal-unconstr}
	\umin{x} F(x) + G(x)
	\qwhereq
	\choice{
	F(x) \eqdef \sum_{k=1}^{N-1} w_i H_{q_k}^*(u_k) 
		+ w_N H_{q_N}^*\pa{  u_N(x) } \\
	G(x) \eqdef J^*(v).
	}
}

We assume that one is able to compute the proximal operator of $J^*$
\eql{\label{eq-proximal-map}
	\Prox_{\tau J^*}(v) = \uargmin{v'} \frac{1}{2}\norm{v-v'}^2 + \tau J^*(v').
}
It is for instance an orthogonal projector on a convex set $C$ when $J^*=\iota_{C}$ is the indicator of $C$. 
%
One can compute easily this projection for instance when $J$ is the $\ell^2$ or the $\ell^1$ norm (see Section~\ref{sec-tv-regul}). 
%
We refer to~\cite{BauschkeCombettes11} for more background on proximal operators. 


The proximal operator of $G$ is then simply
\eq{
	\foralls x=((u_k)_{k=1}^{N-1}, v), \quad \Prox_{\tau G}(x) = ( (u_k)_{k=1}^{N-1}, \Prox_{\tau J^*}(v) ). 
}
Note also that the function $F$ is smooth with a Lipschitz gradient, and that
\eq{
	\nabla F( (u_k)_{k=1}^{N-1}, v ) = 
	\pa{  
		(
			w_k ( \nabla H_{q_k}^*(u_k) 
			-
			\nabla H_{q_N}^*(u_N)  )
		)_{k=1}^{N-1}, 		
		-\Aa \nabla H_{q_N}^*(u_N)
	}
}

The simplest algorithm to solve~\eqref{eq-primal-unconstr} is the Forward-Backward algorithm, whose iteration read
\eql{\label{eq-algo-fb}
	\IIT{x} = \Prox_{\tau J^*}\pa{ \IT{x} - \tau \nabla F(\IT{x}) }.
}
It $\tau<2/L$ where $L$ is the Lipschitz constant of $\nabla F$, then $\IT{x}$ converge to a solution of~\eqref{eq-primal-unconstr}, see~\cite{BauschkeCombettes11} and the references therein. In order to accelerate the convergence of the method, one can use accelerated schemes such as FISTA's algorithm~\cite{beck-fista}. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Total Variation Regularization}
\label{sec-tv-regul}

A typical example of regularization to enforce some geometrical regularity in the barycenter is the total variation regularization on a grid in $\RR^d$ (e.g. $d=2$ for images). It is obtained by considering
\eql{\label{eq-exmp-tv}
	\Aa p \eqdef \nabla p = ( \nabla_i p )_i
	\qandq
	J(u) \eqdef \la \sum_i \norm{u_i}_{\beta}, 
}
where $\nabla_i p \in \RR^d$ is a finite difference approximation of the gradient at a point indexed by $i$, and $\la \geq 0$ is the regularization strength.
%
When using the $\ell^2$ norm to measure the gradient amplitude, i.e. $\beta=2$, one obtains the so-called isotropic total variation, that tends to round corners, and essentially penalizes the length of the level sets of the barycenter, possibly merging clusters together. 
%
When using instead the $\ell^1$ norm, i.e. $\beta=1$, one obtains the so-called anisotropic total variation, which penalizes independently horizontal and vertical derivative, thus favoring the emergence of axis-aligned edges, and giving a ``crystalline'' look to the barycenters. We refer for instance to~\cite{2015-Caselles-tv} for a study of the effect of TV regularization on the shapes of levelsets using isotropic and crystalline total variations. 

In this case, it is possible to compute in closed form the proximal operator~\eqref{eq-proximal-map}. Indeed, one has $J^* = \iota_{\norm{\cdot}_{\beta^*} \leq \la}$ where $\beta^*$ is the conjugate exponent $1/\beta+1/\beta^*=1$. One can compute explicitly the proximal operator in the case $\beta \in \{1,2\}$ since they correspond to orthogonal projectors on $\ell^{\beta^*}$ balls
\eq{
	\Prox_{\tau J^*}(v)_i = 
	\choice{
		\min(\max(v_i,-\la), \la) \qifq \beta=1,  \\
		v_i \frac{\la}{ \max(\norm{v_i},1) }  \qifq \beta=2.
	}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Barycenters of Images}
\label{sec-tv-images}

We start by computing barycenters of a small number of 2-D images, that are discretized on an uniform rectangular grid of $n=256 \times 256$ pixels $(z_i)_{i=1}^N$. We use either the isotropic ($\beta=2$) or anisotropic ($\beta=1$) total variation presented above, where $\nabla$ is defined using standard forward finite differences along each axis, and using Neumann boundary conditions. The metric is the usual squared Euclidean metric
\eql{\label{eq-squared-eucl-metric}
	\foralls (i,j) \in \{1,\ldots,n\}^2, \quad
	M_{i,j} = \norm{z_i-z_j}^2. 
}
The Gibbs kernel $K=e^{-M/\ga}$ is a filtering with a Gaussian kernel, that can be applied efficiently to histograms in nearly linear time, see~\cite{2015-solomon-siggraph} for more details about convolutional kernels. 


\newcommand{\myPic}[3]{\includegraphics[width=.19\linewidth]{tv-regularization/bary4-#1/lambda#2/bary#3}}
\newcommand{\myspace}{\hspace{0mm}}

\newcommand{\myTable}[3]{ % 
	\begin{subfigure}[b]{0.48\textwidth}
	\begin{tabular}{|@{}c@{\myspace{}}c@{\myspace{}}c@{\myspace{}}c@{\myspace{}}c@{}|}
		\hline
		\myPic{#1}{#2}{1}&
		\myPic{#1}{#2}{2}&
		\myPic{#1}{#2}{3}&
		\myPic{#1}{#2}{4}&
		\myPic{#1}{#2}{5}\\[-2mm]
		\myPic{#1}{#2}{6}&
		\myPic{#1}{#2}{7}&
		\myPic{#1}{#2}{8}&
		\myPic{#1}{#2}{9}&
		\myPic{#1}{#2}{10}\\[-2mm]
		\myPic{#1}{#2}{11}&
		\myPic{#1}{#2}{12}&
		\myPic{#1}{#2}{13}&
		\myPic{#1}{#2}{14}&
		\myPic{#1}{#2}{15}\\[-2mm]
		\myPic{#1}{#2}{16}&
		\myPic{#1}{#2}{17}&
		\myPic{#1}{#2}{18}&
		\myPic{#1}{#2}{19}&
		\myPic{#1}{#2}{20}\\[-2mm]
		\myPic{#1}{#2}{21}&
		\myPic{#1}{#2}{22}&
		\myPic{#1}{#2}{23}&
		\myPic{#1}{#2}{24}&
		\myPic{#1}{#2}{25}\\\hline
	\end{tabular}
	\caption{#3}
	\end{subfigure}}

\begin{figure}[h!]
	\centering	
	\myTable{aniso}{0}{$\la=0$}	 
	\myTable{iso}{1000}{Isotropic, $\la=100$}	 
	\myTable{aniso}{500}{Anisotropic $\la=500$}	 
	\myTable{aniso}{2000}{Anisotropic $\la=2000$}	 
	\caption{% 
		Examples of isotropic and anisotropic TV regularization for the computation of barycenters between four input densities. 
		The weights $(w_k)_{k=1}^N$ are bilinear interpolation weights, so that it is for instance $w=(1,0,0,0)$ on the 
		top left corner and $(0,0,0,1)$ on the bottom right corner.  \label{fig-images-bary}
	}
\end{figure}

Figure~\ref{fig-images-bary} shows examples of barycenters of $N=4$ input histograms computed by solving~\eqref{eq-regul-primal} using the projected gradient descent method~\eqref{eq-algo-fb}. The input histograms represent 2-D shapes, and are uniform (constant) distributions inside the support of the shapes. Note that in general the barycenters are not shapes, i.e. they are not uniform distributions, but this method can nevertheless be used to define meaningful averaging of shapes as exposed in~\cite{2015-solomon-siggraph}. 
%
Figure~\ref{fig-images-bary} compares the effects of $\beta \in \{1,2\}$, and one can clearly see how the isotropic total variation ($\beta=2$) rounds the corners of the input densities, while the anisotropic version ($\beta=1$) favors horizontal/vertical edges.  


\newcommand{\myPicL}[2]{\includegraphics[width=.125\linewidth]{tv-regularization/bary2-#1/bary1-lambda#2}}

\begin{figure}[h!]
	\centering	
	\begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
		\myPicL{iso}{0} &
		\myPicL{iso}{200} &
		\myPicL{iso}{400} &
		\myPicL{iso}{600} &
		\myPicL{iso}{800} &
		\myPicL{iso}{1000} &
		\myPicL{iso}{2000} &
		\myPicL{iso}{3000} \\
		\myPicL{aniso}{0} &
		\myPicL{aniso}{200} &
		\myPicL{aniso}{400} &
		\myPicL{aniso}{600} &
		\myPicL{aniso}{800} &
		\myPicL{aniso}{1000} &
		\myPicL{aniso}{2000} &
		\myPicL{aniso}{3000} \\
		$\la=0$ &
		$\la=20$ &
		$\la=40$ &
		$\la=60$ &
		$\la=80$ &
		$\la=100$ &
		$\la=200$ &
		$\la=300$ 
	\end{tabular}	 
	\caption{% 
		Influence of $\la$ parameter for the iso-barycenter (i.e. $w=(1/2,1/2)$) between two input densities (they are the upper-left and upper-right corner of the $\la=0$ case in Figure~\ref{fig-images-bary}). 
		\textit{Top row:} isotropic total variation ($\beta=2$).
		\textit{Bottom row:} anisotropic total variation ($\beta=1$). \label{fig-images-influ-lambda}
	}
\end{figure}

Figure~\ref{fig-images-influ-lambda} shows the influence of the regularization strength $\la$ to compute the iso-barycenter of $N=2$ shapes. This highlights the fact that this total variation regularization has the tendency to group together small clusters, which might be beneficial for some applications, as illustrated in Section~\ref{sec-tv-meg} on MEG data denoising. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Barycenters of MEG Data}
\label{sec-tv-meg}

We applied our method to a magnetoencephalography (MEG) dataset. In this setup, brain activity of a subject is recorded  (Elekta Neuromag, 306 sensors of which 204 planar gradiometers and 102 magnetometers, sampling frequency 1000Hz) while it reacted to the presentation of a target stimulus by pressing either the left or the right button.

Data is preprocessed applying signal space separation correction, interpolation of noisy sensors, and realignment of data into a subject-specific head position (MaxFilter, Elekta Neuromag). The signal was then filtered (low pass 40HZ), and artifacts such as blinks and heartbeats removed thanks to Signal-Space Projection using the Brainstorm software\footnote{\url{http://neuroimage.usc.edu/brainstorm}}. The samples we used for our barycenter computations are an average of the norm of the two gradiometers for each channel from stimulation onto 50ms and the classes were left or right button. 

\newcommand{\myPicMEGin}[2]{\includegraphics[width=.125\linewidth]{meg/input/#1-#2}}
\newcommand{\myPicMEGbar}[2]{\includegraphics[width=.125\linewidth]{meg/bary/bary#1-lambda#2}}
\newcommand{\myPicMEGmean}[1]{\includegraphics[width=.125\linewidth]{meg/bary/bary#1-mean}}


\begin{figure}[h!]
	\centering	
	\begin{tabular}{@{}c@{}c@{}c@{}c@{}|@{}c@{}c@{}c@{}c@{}}
		& Class 1 & & & %
		& Class 2 & & \\ % 
		\myPicMEGin{1}{1} &
		\myPicMEGin{1}{2} &
		\myPicMEGin{1}{3} &
		\myPicMEGmean{1} & 
		%%%%
		\myPicMEGin{2}{1} &
		\myPicMEGin{2}{2} &
		\myPicMEGin{2}{3} &
		\myPicMEGmean{2} \\
		Sample 1 & 
		Sample 2 &
		Sample 3 &
		Mean &
		Sample 1 & 
		Sample 2 &
		Sample 3 &
		Mean  \\
		\myPicMEGbar{1}{0} &
		\myPicMEGbar{1}{2} &
		\myPicMEGbar{1}{4} &
		\myPicMEGbar{1}{8} &
		%%%
		\myPicMEGbar{2}{0} &
		\myPicMEGbar{2}{2} &
		\myPicMEGbar{2}{4} &
		\myPicMEGbar{2}{8} \\
		$\la=0$ &
		$\la=2$ &
		$\la=4$ &
		$\la=8$ &		
		%%%
		$\la=0$ &
		$\la=2$ &
		$\la=4$ &
		$\la=8$ 
	\end{tabular}	 
	\caption{% 
		Barycenter computation on MEG data. The left/right panels shows respectively the first and the second class, 
		corresponding to recordings where the subject is asked to push the left or the right button.
		%
		\textit{Top row:} examples of input histograms $q_k$ for each class, as well as the 
		$\ell^2$ mean $N^{-1} \sum_k q_k$.
		\textit{Bottom row:} computed TV-regularized barycenter for different values of $\la$
		($\la=0$ corresponding to no regularization). \label{fig-meg}
	}
\end{figure}


This results in two classes of recordings, one for each pressed button. We we aim at computing a representative activity map for each class using Wasserstein barycenters. For each class we have $N=33$ recordings $(q_k)_{k=1}^N$ each having $n=66$ samples located on the vertices an hexahedral mesh of an hemisphere (corresponding to a MEG recording helmet). These recorded values are positive by construction, and we rescale them linearly to impose $q_k \in \Si_n$.  Figure~\ref{fig-meg}, top row, shows some samples from this dataset, displayed using interpolated colors as well as iso-level curves. The black dots represent the position $(z_i)_{i=1}^n$ of the electrode on the half-sphere of the helmet, flattened on a 2-D disk. 

We computed TV-regularized barycenters independently for each class by solving~\eqref{eq-regul-primal} with the TV regularization using the projected gradient descent method~\eqref{eq-algo-fb}. We used a squared Euclidean metric~\eqref{eq-squared-eucl-metric} on the flattened hemisphere.
%
Since the data is defined on an irregular graph, instead of~\eqref{eq-exmp-tv}, we use a graph-based discrete gradient. We denote $( (i,j) )_{(i,j) \in \Gg}$ the graph which connects neighboring electrodes. The gradient operator on the graph is
\eq{
	\foralls p \in \RR^n, \quad
	\Aa p \eqdef ( p_i - p_j )_{ (i,j) \in \Gg } \in \RR^{|\Gg|}.
}
The total variation on this graph is then obtained by using $J = \la \norm{\cdot}_1$, the $\ell^1$ norm, i.e. we use $\beta=1$ in~\eqref{eq-exmp-tv}. 

Figure~\ref{fig-meg} compares the naive $\ell^2$ barycenters (i.e. the usual mean), barycenters obtained without regularization (i.e. $\la=0$) and barycenters computed with an increasing regularization strength $\la$. The input histograms $(p_k)_k$ being very noisy, the use of regularization is important to make the area of significant activity emerge from the noise. The use of a TV regularization helps to keep a sharp transition between active and non-active regions. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Gradient Flow}

Instead of computing barycenters, we now use our regularization to define time-evolutions, which are defined through a so-called discrete gradient flow. 

Starting from an initial histogram $p_0 \in \Si_n$, we define iteratively 
\eql{\label{eq-gradflow-def}
	p_{k+1} \eqdef \uargmin{p \in \Si_N} H_{p_k}(p) + \tau f(p).
}
This means that one seeks a new iterate at (discrete time) $k+1$ that is both close (according to the Wasserstein distance) to $p_k$ and minimizes the functional $f$. In the following, we consider the gradient flow of regularization functionals as considered before, i.e. that are of the form $\tau f = J \circ \Aa$. Problem~\eqref{eq-gradflow-def} is thus a special case of~\eqref{eq-regul-primal} with $N=1$. 

Letting $k \rightarrow +\infty$, one can informally think of $p_k$ as a discretization of a time evolution evaluated at time $t=k\tau$. This method is a general scheme presented in detail in the monograph~\cite{ambrosio2006gradient}. The use of an implicit time-stepping~\eqref{eq-gradflow-def} allows one to define time evolutions to minimize functionals that are not necessarily smooth, and this is exactly the case of the total variation semi-norm (since $J$ is not differentiable). 
%
The use of gradient flows in the context of the Wasserstein fidelity to the previous iterate has been introduced initially in the seminal paper~\cite{jordan1998variational}. When $f$ is the entropy functional, this paper proves that the countinous flow defined by the limit $k \rightarrow+\infty$ is a heat equation. Numerous theoretical papers have shown how to recover many existing non-linear PDE's by considering the appropriate functional $f$, see for instance~\cite{otto2001geometry,GianazzaARMA}.

The numerical method we consider in this article is the one introduced in~\cite{Peyre-JKO}, that makes use of the entropic smoothing of the Wasserstein distance. It is not the scope of the present paper to discuss the problem of approximating gradient flows and the underlying limit non-linear PDE's, and we refer to~\cite{Peyre-JKO} for an overview of the vast literature on this topic. A major bottleneck of the algorithm developed in~\cite{Peyre-JKO} is that it uses a primal optimization scheme (Dykstra's algorithm) that necessitates the computation of the proximal operator of $f$ according to the Kulback-Leibler divergence. Only relatively simple functionals (basically separable functionals such as the entropy) can thus be treated by this approach. In contrast, our dual method can cope with a much larger set of functions, and in particular those of the form $f = J \circ \Aa$, i.e. obtained by pre-composition with a linear operator. 


\newcommand{\myPicGF}[2]{\includegraphics[width=.16\linewidth]{gradient-flow/#1/#1-flow-#2}}

\begin{figure}[h!]
	\centering	
	\begin{tabular}{@{}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{}}
		\myPicGF{randdisks}{0} &
		\myPicGF{randdisks}{2} &
		\myPicGF{randdisks}{5} &
		\myPicGF{randdisks}{10} &
		\myPicGF{randdisks}{15} &
		\myPicGF{randdisks}{20}  \\
		\myPicGF{hibiscus}{0} &
		\myPicGF{hibiscus}{2} &
		\myPicGF{hibiscus}{5} &
		\myPicGF{hibiscus}{10} &
		\myPicGF{hibiscus}{15} &
		\myPicGF{hibiscus}{20}  \\
		$t=0$ &
		$t=20$ &
		$t=40$ &
		$t=60$ &
		$t=80$ &
		$t=100$ 
	\end{tabular}	 
	\caption{% 
		Examples of gradient flows~\eqref{eq-gradflow-def} at various times $t \eqdef k\tau$. \label{fig-gradient-flow}
	}
\end{figure}


Figure~\ref{fig-gradient-flow} shows examples of gradient flows computed for the isotropic total variation $f(p)=\norm{\nabla p}_1$ as defined in~\eqref{eq-exmp-tv}. We use the discretization setup considered in Section~\ref{sec-tv-images}. This is exactly the regularization flow considered by~\cite{Burger-JKO}. This paper formally derives the highly non-linear fourth order PDE corresponding to the limit flow. This is however not a ``true'' PDE since the initial TV functional is non-smooth, and derivative should be understood in a weak sense, as limit of an implicit discrete time stepping. While the algorithm proposed in~\cite{Burger-JKO} uses the usual (unregularized) Wasserstein distance, the use of a regularized transport, thanks to the connexion with Gaussian filtering, allows us to deal with larger problems, in 2-D, with a faster numerical scheme. The price to pay is an additional blurring introduced by the  entropic smoothing, but this is acceptable for applications to denoising in imaging. Figure~\ref{fig-gradient-flow} illustrates the behavior of this TV regularization flow, which has the tendency to group together clusters of mass, and performs some kind of progressive ``percolation'' over the whole image. 





